New refiners for permutation group search

We describe how orbital graphs can be used to improve the practical performance of many algorithms for permutation groups, including intersection and stabilizer problems. First we explain how orbital graphs can be integrated in partition backtracking, the current state of the art algorithm for many permutation group problems. We then show how our algorithms perform in practice, demonstrating improvements of several orders of magnitude for some problems.

==> implement.tex <==
\subsubsection{Implementation}

In this section we will show how to find the orbital graphs of a group \(G\), skipping the pointless ones. We will assume the existence of

The technique we use for finding orbitals is given in \cref{alg:orbitals}. This algorithm assumes the use of a computational group theory system such as GAP which provides a number of basic group theory algorithms, in particular finding orbits of points and pairs of points, and point stabilizers.

\begin{algorithm}
\caption{Find Orbital Graphs}\label{alg:orbitals}
\begin{algorithmic}[1]
\Procedure{OrbitalBase}{$G,\Omega, SizeLimit$}\Comment{Orbital graphs of \(G\), a perm group on \(\Omega\)}
  \State{\(\mathrm{Graphs} := []\)}
  \For{\(Orb \in \mathrm{Orbits}(G)\)}
    \If{\(|Orb| > 1\)}\label{line:if-basic}
   	  \State \(G' = \mathrm{Stabilizer}(G, \mathrm{Min}(Orb))\)
	  \For{\(InnerOrb \in\) Orbits\((G')\)}
	     \If{\(|\mathrm{Orb}|\times |\mathrm{InnerOrb}| \leq SizeLimit\)}\label{line:if-sizelimit}
        \If{\(InnerOrb \not\in \mathrm{Orbits}(G)\)}\label{line:if-bipartite}
        \If{\(!(InnerOrb \not\in Orb \vee |InnerOrb| + 1 \neq |Orb|)\)}\label{line:if-clique}

          \State \(\mathrm{Add}(Graphs, Orbit(G, \la \mathrm{Min}(Orb), \mathrm{Min}(InnerOrb) \ra ) )\)
		\EndIf\EndIf\EndIf
	  \EndFor
    \EndIf
  \EndFor
  \State \Return{Graphs}
\EndProcedure
\end{algorithmic}
\end{algorithm}

Except for \cref{line:if-basic,line:if-bipartite,line:if-clique,line:if-sizelimit}, \cref{alg:orbitals} finds all orbital graphs in a standard manner. \Cref{line:if-basic} only provides a simple optimisation as when the size of Orb is 1, then \(G' = G\) and therefore \(InnerOrb \in \mathrm{Orbits}(G)\), and so \cref{line:if-bipartite} would be false.

The correctness of  \cref{line:if-bipartite,line:if-clique,line:if-sizelimit} rely on the fact we can easily calculate the size of an orbital graph without explicitly creating it. A proof of this result is given in \cref{lem:orbitalsize}.

\begin{lem}\label{lem:orbitalsize}
Given a permutation group \(G\) on a set \(\Omega\) and two points \(a,b \in \Omega\), then the number of edges in the orbital graph of the directed pair \(\la a,b\ra\) in \(G\) is equal to the size of the orbit of \(a\) in \(G\) multiplied by the size of the orbit of \(b\) in \(\mathrm{Stabilizer}(G,a)\).
\end{lem}

\begin{proof}
\textbf{This seems almost too obvious to both proving?}
The number of edges whose first member is \(a\) in the orbital of \(\la a,b\ra\) is the size of the orbit of \(b\) in \(\mathrm{Stabilizer}(G,a)\). For each image of \(a\) in \(G\), there will be a distinct image of each of these edges.
\end{proof}

When we look at the orbital graphs of a group \(G\), we can divide them into two classes, the anti-symmetric ones (where there is no edge and its inverse) and the symmetric ones (where there is at least one edge and its inverse). Once the graph contains an edge, and its inverse, it must contain  graph contains the inverse of every edge in the revery edge is paired with its inthere exists no pair of edges of the form \(\la a,b\ra\) and \(\la b,\)

\textbf{I leave these lemmas, but I might not want them}

\begin{lem}
Consider a group \(G\) of \(\Omega\) which can be expressed as \(Sym_P\) for some ordered partition \(P\) of \(\Omega\). Then the orbital graphs of \(G\) take two forms:

\begin{enumerate}
\item Given a directed edge \((x,y,i)\) where \(x\) and \(y\) lie with the same cell of \(P\), the orbital graph is the \textbf{clique graph} on \(S_i\).
\item Given a directed edge \((x,y,i)\) where \(x\) lives in cell \(i\) and \(y\) lies in cell \(j\), for \(i \neq j\), the orbital graph is the \textbf{directed bipartite graph} between cells \(P_i\) and \(P_j\).
\end{enumerate}
\end{lem}

\begin{proof}
These constructions follow directly from the definitions of clique and directed bipartite graphs.
\begin{enumerate}
\item The image of the ordered pair \((x,y)\) under the symmetric group on \(S_i\) is all pairs \(i,j\) where \(\{i,j\} \subseteq P\)
\item The images of the ordered pair \((x,y)\) under the symmetric group on \(P_i\) (which contains \(x\)) and the symmetric group on \(P_j\) (which contains \(y\)) is the set \(E = \{(x,y) | x \in P_i, y \in P_j\)
\end{enumerate}
\end{proof}


\begin{lem}
The automorphism groups of \textbf{clique graphs} and a \textbf{directed bipartite graphs} are a direct product of symmetric groups.
\end{lem}

\begin{proof}
Firstly, consider a clique graph \(G=V,E\) with a clique on the set of vertices \(C \subseteq V\). Then any automorphism of \(G\) may permute vertices in \(C\), and also permute vertices not in \(C\), but may not swap any vertex in \(C\) with a vertex not in \(C\). Therefore the automorphism group is exactly \(Sym_{S_C} x Sym_{S_{V-C}}\).

Secondly, consider a directed bipartite graph \(G=V,E\) on the two disjoint subsets of vertices \(C,D \subseteq V\), with edges mapping \(C\) to \(D\). As the only vertices with edges leaving are in \(C\), then automorphisms of \(G\) cannot map vertices in \(C\) to vertices outside \(C\), and similarly for \(D\). As there are all edges between \(C\) and \(D\), the automorphisms are therefore exactly \(Sym_{S_C} x Sym_{S_D} x Sym_{S_{V-D-C}}\).
\end{proof}



